What Causes Exceptions in Machine Learning Applications? Mining Machine Learning-Related Stack Traces on Stack Overflow

Machine learning (ML), including deep learning, has recently gained tremendous popularity in a wide range of applications. However, like traditional software, ML applications are not immune to the bugs that result from programming errors. Explicit programming errors usually manifest through error messages and stack traces. These stack traces describe the chain of function calls that lead to an anomalous situation, or exception. Indeed, these exceptions may cross the entire software stack (including applications and libraries). Thus, studying the patterns in stack traces can help practitioners and researchers understand the causes of exceptions in ML applications and the challenges faced by ML developers. To that end, we mine Stack Overflow (SO) and study 11,449 stack traces related to seven popular Python ML libraries. First, we observe that ML questions that contain stack traces gain more popularity than questions without stack traces; however, they are less likely to get accepted answers. Second, we observe that recurrent patterns exists in ML stack traces, even across different ML libraries, with a small portion of patterns covering many stack traces. Third, we derive five high-level categories and 25 low-level types from the stack trace patterns: most patterns are related to python basic syntax, model training, parallelization, data transformation, and subprocess invocation. Furthermore, the patterns related to subprocess invocation, external module execution, and remote API call are among the least likely to get accepted answers on SO. Our findings provide insights for researchers, ML library providers, and ML application developers to improve the quality of ML libraries and their applications.

==> Table/tbl_patterns.tex <==
\begin{table}[]
    \centering
    \vspace{4mm}
    \small
    \renewcommand{\arraystretch}{1.2} % adds row cushion
    \caption{Post w/o repetitive pattern - most questions has pattern)}
    \begin{adjustbox}{width=0.6\linewidth, center}
    \begin{tabular}{lrr}
    \toprule
         \textbf{ML Libraries} & \textbf{\#~Lost Posts} & \textbf{Percentage (\%)}\\ 
        \hline
        \rowcolor{gray!15}
        \multicolumn{1}{l||}{TensorFlow} & 464 & 8.55 \\
        \multicolumn{1}{l||}{Keras} & 296 & 10.91 \\
        \rowcolor{gray!15}
        \multicolumn{1}{l||}{Scikit-learn} & 239 & 14.61 \\
        \multicolumn{1}{l||}{PyTorch} & 125 & 17.56 \\
        \rowcolor{gray!15}
        \multicolumn{1}{l||}{NLTK} & 126 & 22.42 \\
        \multicolumn{1}{l||}{Hugging Face} & 13 & 32.50\\
        \rowcolor{gray!15}
        \multicolumn{1}{l||}{Spark ML} & 1 & 6.25\\  
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\label{tab:table25}
\end{table}



==> Table/tmp_tables.tex <==
% \begin{table}[]
% {
%     \centering
%     \small
%     \caption{Number of posts based on several categories}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l| c | c | c}
%         \toprule
        
%         \multirow{2}*{\textbf{ML Framework}} & \multirow{2}*{\textbf{\#~Post}} & \multirow{2}*{\textbf{\#~Code Blocks}} & \multirow{2}*{\textbf{\#~Stack Trace}}\\
%         & & &\\
%         \midrule
        
%         TensorFlow & 39,690 & -- & \textbf{--} \\
%         \rowcolor{gray!15}
%         Keras & 21,568 & 41,764 & \textbf{2,715} \\
%         Scikit-learn & 18,133 & -- & \textbf{--} \\
%         \rowcolor{gray!15}
%         PyTorch & 5,540 & -- & \textbf{--}  \\
%         NLTK & 5,592 & -- & \textbf{--} \\
%         \rowcolor{gray!15}
%         Hugging Face & 236 & -- & \textbf{--}  \\
%         Spark ML & 141 & -- & \textbf{--} \\

%         \bottomrule
        
%     \end{tabular}
%     \end{adjustbox}

% }
% \label{tab:table5}
% \end{table}

% \begin{table*}[]
% {
%     \centering
%     \small
%     \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{Number of posts based on several categories}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l||r|cc|r|cc|rc|cc}
%         % \toprule
%         \multirow{2}*{\textbf{ML Framework}} & \multirow{2}*{\textbf{\#~Post}} & \multicolumn{2}{c|}{\textbf{Post}} & \multirow{2}*{\textbf{\#~Code Blocks}} &
%         \multicolumn{2}{c|}{\textbf{With Code Block}} &  \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{\#~Stack Trace}}} &
%         \multicolumn{2}{c}{\textbf{With Stack Trace}} \\
%         & & with code block & w/o code block & & with stack trace & w/o stack trace & & & Unix OS & Windows OS \\
%         \midrule
%         \rowcolor{gray!15}

%         TensorFlow & 39,690 & 81.6\% & 18.4\% & 70,621 & 16.8\% & 83.2\% & \multicolumn{1}{r:}{\textbf{ 5436 }} & 13.7\% & 69.1\% & 30.9\%
%         \\
%         Keras & 21,568 & 85.8\% & 14.2\% & 41,764 & 14.7\% & 85.3\% & \multicolumn{1}{r:}{\textbf{ 2715 }} & 12.6\% & 70.8\% & 29.2\% \\
%         \rowcolor{gray!15}
%         Scikit-learn & 18,133 & 81.6\% & 18.4\% & 31,293 & 13.6\% & 86.4\% & \multicolumn{1}{r:}{\textbf{ 2009 }} & 11.1\% & 62.0\% & 38.0\% \\
%         PyTorch & 5,540 & 83.4\% & 16.6\% & 9,925 & 15.4\% & 84.6\% & \multicolumn{1}{r:}{\textbf{ 713 }} & 12.9\% & 76.2\% & 23.8\% \\
%         \rowcolor{gray!15}
%         NLTK & 5,592 & 78.3\% & 21.7\% & 8,999 & 12.9\% & 87.1\% & \multicolumn{1}{r:}{\textbf{ 564 }} & 10.1\% & 58.7\% & 41.3\% \\
%         Hugging Face & 236 & 86.4\% & 13.6\% & 460 & 19.6\% & 80.4\% & \multicolumn{1}{r:}{\textbf{ 40 }} & 16.9\% & 87.5\% & 12.5\% \\
%         \rowcolor{gray!15}
%         Spark ML & 141 & 89.4\% & 10.6\% & 323 & 12.7\% & 87.3\% & \multicolumn{1}{r:}{\textbf{ 16 }} & 11.3\% & 100.0\% & -- \\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% }
% \label{tab:table1}
% \end{table*}

% \begin{table*}[]
% {
%     \centering
%     \small
%     \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{Modified - Number of posts based on several categories}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l||r|rc|rc|cc}
%         % \toprule
%         \multirow{2}*{\textbf{ML Libraries}} & \multirow{2}*{\textbf{\#~Posts}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{\#~Posts with code block}}} &  \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{\#~Posts with stack trace}}} & \multicolumn{2}{c}{\textbf{OS$^1$}} \\
%         & & & & & & Unix-based & Windows \\
%         \midrule
%         \rowcolor{gray!15}
%         TensorFlow & 39,690 &  \multicolumn{1}{r:}{32,368} & 81.6\% & \multicolumn{1}{r:}{\textbf{ 5,436 }} & 13.6\% & 69.1\% & 30.9\% \\
%         Keras & 21,568 & \multicolumn{1}{r:}{18,506} & 85.8\% & \multicolumn{1}{r:}{\textbf{ 2,715 }} & 12.5\% & 70.8\% & 29.2\% \\
%         \rowcolor{gray!15}
%         Scikit-learn & 18,133 & \multicolumn{1}{r:}{14,795} & 81.6\% & \multicolumn{1}{r:}{\textbf{ 2,009 }} & 11.0\% & 62.0\% & 38.0\% \\
%         PyTorch & 5,540 & \multicolumn{1}{r:}{4,620} & 83.4\% & \multicolumn{1}{r:}{\textbf{ 713 }} & 12.8\% & 76.2\% & 23.8\% \\
%         \rowcolor{gray!15}
%         NLTK & 5,592 & \multicolumn{1}{r:}{4,381} & 78.3\% & \multicolumn{1}{r:}{\textbf{ 564 }} & 10.0\% & 58.7\% & 41.3\% \\
%         Hugging Face & 236 & \multicolumn{1}{r:}{204} & 86.4\% & \multicolumn{1}{r:}{\textbf{ 40 }} & 16.9\% & 87.5\% & 12.5\% \\
%         \rowcolor{gray!15}
%         Spark ML & 141 & \multicolumn{1}{r:}{126} & 89.4\% & \multicolumn{1}{r:}{\textbf{ 16 }} & 11.3\% & 100\% & -- \\
%         \bottomrule
%         \multicolumn{7}{l}{\small $^1$ OS stands for ... (OS used to generate st)} \\
%     \end{tabular}
%     \end{adjustbox}
% }
% \label{tab:table1}
% \end{table*}


% \begin{table}[]
%     \centering
%     \small
%     \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{Answer Duration\xam{Something is weird with p-value for HuggingFace}}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|rrrrrr}
%         \toprule
%         \multicolumn{1}{c}{\multirow{3}{*}{}} & \multicolumn{6}{c}{\textbf{The Median of Answer Duration}} \\ \cmidrule(l){2-7} 
%         \multicolumn{1}{c}{}  & \multicolumn{3}{c}{First Answer (Hour)} & \multicolumn{3}{c}{First Accepted Answer (Hour)} \\ \cmidrule(l){2-4}\cmidrule(l){5-7}
%         \multicolumn{1}{c}{\textbf{ML Framework}}  & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-value} \\ \midrule
%         \rowcolor{gray!15}
%         TensorFlow & 5.82 & 1.88 & 4.22e-75 & 3.96 & 2.40 & 2.019e-08 \\
%         Keras & 3.27 & 1.86 &4.673e-12& 2.24 & 1.84& 0.0048\\
%         \rowcolor{gray!15}
%         Scikit-learn & 2.97 & 1.53 &7.92e-14& 2.50 & 1.56& 2.576e-07\\
%         PyTorch & 4.10 & 2.53 & 0.0007 & 3.08 & 2.53& 0.1117 \\
%         \rowcolor{gray!15}
%         NLTK & 2.39 & 1.14 & 0.0001 & 2.91 & 1.16& 0.0010\\
%         Hugging Face & 21.24 & 18.48 & 0.353 & 0.98 & 14.10 & 0.105\\
%         \rowcolor{gray!15}
%         Spark ML & 2.40 & 2.43 & 0.870 & 1.97 & 1.79& 0.958 \\ \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table2}
% \end{table}
% \begin{tcolorbox}
%     \textbf{What is the percentage of questions?}\\
%     We captured 163194 posts on SOTorrent related to the ML topics and filtered 61338 questions containing the TensorFlow tag. Table~\ref{tab:number} indicates all specifications about these questions. In detail, "With code" and "W/O Code" columns refer to posts that have or doesn't have code tags inside themself, and we divided code posts again into two groups, questions that contain stack traces or not.
% \end{tcolorbox}
    
% \begin{tcolorbox}
%     \textbf{What is the line of code (LOC) status amongst posts with code tags?}\\
%     Figure~\ref{fig:loc} indicates our results comparing the LOC in posts containing regular snippet codes and stack traces.
% \end{tcolorbox}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.5\textwidth]{Figure/loc.pdf}
%   \caption[Short text]{Comparing the LOC between regular code and stack trace}
%   \label{fig:loc}
% \end{figure}

%  \begin{tcolorbox}
%     \textbf{What is the status of question length between posts with and without stack traces?}\\
%     We count the number of words for each question body to answer this question. Figure~\ref{fig:q_length} illustrates the result of this investigation. We can find that the statistical parameters (e.g., mean) are approximately the same in both situations.
% \end{tcolorbox} 

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.5\textwidth]{Figure/Q_length.pdf}
%   \caption[Short text]{Comparing the Question Length}
%   \label{fig:q_length}
% \end{figure}


%  \begin{tcolorbox}
%     \textbf{What's the average time of question to get an answer?}\\
%     Figures~\ref{fig:ans1} and ~\ref{fig:ans2} show the duration of first and accepted answers in posts that have and don't have stack traces, respectively.
% \end{tcolorbox}   

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.5\textwidth]{Figure/answer_count.pdf}
%   \caption[Short text]{Answers Duration (with stack traces)}
%   \label{fig:ans1}
% \end{figure}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.45\textwidth]{project report/ans1.png}
%   \caption[Short text]{Answers Duration (w/o stack traces)}
%   \label{fig:ans2}
% \end{figure}


% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.5\textwidth]{Figure/score.pdf}
%   \caption[Short text]{Score Count}
%   \label{fig:sc}
% \end{figure}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.5\textwidth]{Figure/comment.pdf}
%   \caption[Short text]{Comment Count}
%   \label{fig:cc}
% \end{figure}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.45\textwidth]{Figure/answer_count.pdf}
%   \caption[Short text]{Answer Count\xam{something seems odd with the median lines, seems like some should be higher. right now they are all at exactly the middle of the largest bump, even when some distributions have long tails...}}
%   \label{fig:ac}
% \end{figure}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=.45\textwidth]{Figure/view.pdf}
%   \caption[Short text]{View Count}
%   \label{fig:vc}
% \end{figure}

% \begin{table}[]
%     \centering
%     \small
%     \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{The Median of Answer Duration }
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|rclrcl}
%         % \toprule
%         % \multicolumn{1}{c}{\multirow{3}{*}{}} & \multicolumn{6}{c}{\textbf{The Median of Answer Duration}} \\ \cmidrule(l){2-7} 
%         \multicolumn{1}{c}{}  & \multicolumn{3}{c}{First Answer (Hour)} & \multicolumn{3}{c}{Accepted Answer (Hour)} \\ \cmidrule(l){2-4}\cmidrule(l){5-7}
%         \multicolumn{1}{c}{\textbf{ML Libraries}}  & with stack trace & w/o stack trace & \multicolumn{1}{c}{Sig.$^1$} & with stack trace & w/o stack trace & \multicolumn{1}{c}{Sig.} \\ \midrule
%         \rowcolor{gray!15}
%         TensorFlow & 3.09 & 3.04 & o & 2.57 & 2.86 & o\\
%         Keras & 2.00 & 1.66 & *** & 1.88 & 1.60 & *\\
%         \rowcolor{gray!15}
%         Scikit-learn & 1.63 & 1.94 & o & 1.63 & 2.17 & **\\
%         PyTorch & 2.69 & 2.44 & o & 2.63 & 2.45 & o \\
%         \rowcolor{gray!15}
%         NLTK & 1.22 & 2.29 & *** & 1.22 & 2.88 & ***\\
%         Hugging Face & 19.44 & 9.64 & o & 12.92 & 5.03 & o\\
%         \rowcolor{gray!15}
%         Spark ML & 2.43 & 2.83 & o & 1.79 & 3.57 & o \\ \bottomrule
%         \multicolumn{7}{l}{\small $^1$ o $ p \ge 0.05 $; * $ p < 0.05 $; ** $ p < 0.01 $; *** $ p < 0.001$} \\
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table2}
% \end{table}

% \begin{table*}[h]
%     \centering
%     \small
%     \caption{All}
%     \begin{adjustbox}{width=1\linewidth, center}
%         \begin{tabular}{l||lccllccllccllccl}
%         \toprule
%         \multicolumn{1}{c||}{\multirow{2}{*}{ML Framework}} &  & \multicolumn{3}{c}{\textbf{Score}} &  & \multicolumn{3}{c}{\textbf{Comment}} &  & \multicolumn{3}{c}{\textbf{View}} &  & \multicolumn{3}{c}{\textbf{Answer Count}} \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} \cmidrule(lr){11-13} \cmidrule(l){15-17} 
%         \multicolumn{1}{c||}{} &  & with stack trace & w/o stack trace & P-Value &  & with stack trace & w/o stack trace & P-Value &  & with stack trace & w/o stack trace & P-Value &  & with stack trace & w/o stack trace & P-Value \\ \cmidrule(r){1-1} \cmidrule(lr){3-5} \cmidrule(lr){7-9} \cmidrule(lr){11-13} \cmidrule(l){15-17} 
%         TensorFlow &  & 1 & 1 &  &  & 0 & 0 &  &  & 518.0 & 361.0 &  &  & 1 & 1 &  \\
%         \rowcolor{gray!15}
%         Keras &  & 1 & 1 &  &  & 0 & 0 &  &  & 432.0 & 269.0 &  &  & 1 & 1 &  \\
%         Scikit-learn &  & 1 & 1 &  &  & 1 & {\ul 1} &  &  & 757.0 & 501.5 &  &  & 1 & 1 &  \\
%         \rowcolor{gray!15}
%         PyTorch &  & 1 & 1 &  &  & 0 & 0 &  &  & 498.5 & 286.5 &  &  & 1 & 1 &  \\
%         NLTK &  & 1 & 1 &  &  & 1 & {\ul 1} &  &  & {\ul 902.5} & 513.0 &  &  & 1 & 1 &  \\
%         \rowcolor{gray!15}
%         Hugging Face &  & 0 & 1 &  &  & {\ul 2} & 0 &  &  & 195.0 & 217.0 &  &  & 1 & 1 &  \\
%         Spark ML &  & {\ul 2} & {\ul 2} &  &  & 0 & 0 &  &  & 739.5 & {\ul 1026.0} &  &  & 1 & 1 &  \\ \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \label{tab:table3}
% \end{table*}

% \begin{table*}[]
%     \centering
%     \small
%     \caption{All}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|ccrccrccrccr}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Score}} & \multicolumn{3}{c}{\textbf{Comment}} & \multicolumn{3}{c}{\textbf{View}} & \multicolumn{3}{c}{\textbf{Answer Count}} \\ \cmidrule(rl){2-4}\cmidrule(rl){5-7}\cmidrule(rl){8-10}\cmidrule(rl){11-13}
%         \multicolumn{1}{c}{\textbf{ML Framework}} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} \\ \midrule
%         \rowcolor{gray!15}
%         TensorFlow & 0 & 1 & 0.001 & 1 & 0 & 1.7923e-11 & 324.0 & 202.0 & 3.21e-51 & 1 & 1 & 0.002  \\
%         Keras & 1 & 0 & 0.394 & 1 & 1 & 0.002 & 282.0 & 162.0 & 1.437e-30 & 1 & 1 & 0.595 \\
%         \rowcolor{gray!15}
%         Scikit-learn & 1 & 1 & 0.471 & 2 & 1 & 1.0207e-20 & 562.0 & 360.5 & 3.7132e-18 & 1 & 1 & 0.0001 \\
%         PyTorch & 0 & 1 & 0.006 & 0 & 0 & 0.041 & 345.0 & 168.0 & 6.6718e-14 & 1 & 1 & 0.209 \\
%         \rowcolor{gray!15}
%         NLTK & 1 & 1 & 0.014 & 2 & 1 & 0.0001 & 651.5 & 394.0 & 3.0124e-14 & 1 & 1 & 0.685 \\
%         Hugging Face & 0 & 0 & 0.192 & 2 & 0 & 0.002 & 134.0 & 131.5 & 0.900 & 1 & 1 & 0.212 \\
%         \rowcolor{gray!15}
%         Spark ML & 1.5 & 1 & 0.893 & 0 & 0 & 0.531 & 597.5 & 651.0 & 1.0 & 1 & 1 & 0.880 \\ \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table3}
% \end{table*}

% \begin{table*}[]
%     \centering
%     \small
%     \caption{All-modified\amin{Do you think the bold values are correct and normal?}}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|ccrccrccrccr}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Score}} & \multicolumn{3}{c}{\textbf{Comment}} & \multicolumn{3}{c}{\textbf{View}} & \multicolumn{3}{c}{\textbf{Answer Count}} \\ \cmidrule(rl){2-4}\cmidrule(rl){5-7}\cmidrule(rl){8-10}\cmidrule(rl){11-13}
%         \multicolumn{1}{c}{\textbf{ML Framework}} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} \\ \midrule
%         \rowcolor{gray!15}
%         TensorFlow & 0 & 1 & $ p < 0.001 $ & 1 & 0 & $ p < 0.001 $ & 324.0 & 202.0 & $ p < 0.001 $ & 1 & 1 & $ p < 0.01 $   \\
%         Keras & 1 & 0 & $ p \ge 0.05 $ & 1 & 1 & $ p < 0.01 $  & 282.0 & 162.0 & $ p < 0.001 $ & 1 & 1 & \textbf{0.595} \\
%         \rowcolor{gray!15}
%         Scikit-learn & 1 & 1 & $ p \ge 0.05 $ & 2 & 1 & $ p < 0.001 $ & 562.0 & 360.5 & $ p < 0.001 $ & 1 & 1 & $ p < 0.001 $ \\
%         PyTorch & 0 & 1 & $ p < 0.01 $ & 0 & 0 & $ p < 0.05 $ & 345.0 & 168.0 & $ p < 0.001 $ & 1 & 1 & $ p \ge 0.05 $ \\
%         \rowcolor{gray!15}
%         NLTK & 1 & 1 & $ p < 0.05 $ & 2 & 1 & $ p < 0.001 $ & 651.5 & 394.0 & $ p < 0.001 $ & 1 & 1 & \textbf{0.685} \\
%         Hugging Face & 0 & 0 & $ p \ge 0.05 $ & 2 & 0 & $ p < 0.01 $ & 134.0 & 131.5 & \textbf{0.900} & 1 & 1 & $ p \ge 0.05 $ \\
%         \rowcolor{gray!15}
%         Spark ML & 1.5 & 1 & \textbf{0.893} & 0 & 0 & \textbf{0.531} & 597.5 & 651.0 & \textbf{1.0} & 1 & 1 & \textbf{0.880} \\ \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table3}
% \end{table*}

% \begin{table}[]
%     \centering
%     % \vspace{4mm}
%     \small
%     \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{Show the difference between the median of ML libraries and the overall population posts on Stack Overflow}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|cccc}
%     \toprule
%         \multicolumn{1}{l|}{\textbf{Tag Category}} & \textbf{Q-Score} & \textbf{Comment Count} & \multicolumn{1}{l}{\textbf{View}} & \multicolumn{1}{l}{\textbf{Answer Count}} \\ 
%         % \cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}
%         \hline
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{Overall} & 0 & 1 & 341.0 & 1 \\
%         \multicolumn{1}{l|}{ML Library} & 1 & 0.5 & 273.5 & 1 \\
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{ML Library (with stack trace)} & 1 & 1 & 345.0 & 1 \\
%         \multicolumn{1}{l|}{ML Library (w/o stack trace)} & 1 & 0 & 202.0 & 1 \\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table3}
% \end{table}

% \begin{table}[]
%     \centering
%     % \vspace{4mm}
%     \small
%     % \renewcommand{\arraystretch}{1.2} % adds row cushion
%     \caption{Length}
%     \begin{adjustbox}{width=1\linewidth, center}
%     \begin{tabular}{l|ccrccr}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Text Length (QL)}} & \multicolumn{3}{c}{\textbf{Code Length (LOC)}} \\ \cmidrule(rl){2-4}\cmidrule(rl){5-7}
%         \multicolumn{1}{c}{\textbf{ML Libraries}} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} & with stack trace & w/o stack trace & \multicolumn{1}{c}{P-Value} \\ \midrule
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{TensorFlow} & 69.0 & 84.0 & 1.8431e-87 & 27.0 & 22.0 & 1.474e-63 \\
%         \multicolumn{1}{l|}{Keras} & 73.0 & 86.0 & 1.564e-35 & 27.0 & 25.0 & 2.54e-07 \\
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{Scikit-learn} & 67.0 & 79.0 & 2.644e-27 & 21.0 & 17.0 & 3.625e-36 \\
%         \multicolumn{1}{l|}{PyTorch} & 68.0 & 77.0 & 1.483e-05 & 20.0 & 20.0 & 0.041 \\
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{NLTK} & 61.0 & 72.0 & 1.6486e-08 & 16.0 & 13.0 & 6.03e-08 \\
%         \multicolumn{1}{l|}{Hugging Face} & 67.5 & 90.0 & 0.020 & 21.0 & 18.5 & 0.307 \\
%         \rowcolor{gray!15}
%         \multicolumn{1}{l|}{Spark ML} & 83.5 & 80.0 & 0.917 & 44.0 & 19.0 & 0.001 \\ \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \label{tab:table3}
% \end{table}


